Langlands Dualities through Bethe/Gauge Correspondence for 3d Gauge Theories

For non-simple laced Lie algebras, the $\text{B}_{N}$ and $\text{C}_{N}$ are Langlands dual to each other in mathematical. In this article, we give another Bethe/Gauge correspondence between 3d (or 2d) classical Lie group supersymmetry gauge theory with closed and open $\text{XXZ}$ (or $\text{XXX}$) spin chain. Here, the representations of the $\text{ADE}$ Lie algebras are self-dual, and while for the non-simple laced Lie algebras $\text{B}_{N}$ and $\text{C}_{N}$, their roles are exchanged in contrast with the results in \cite{DZ23a}. From Bethe/Gauge correspondence point of view, the two types of the effective superpotentials are Langlands duality to each other. For the $\text{B}_{N}$-type Lie algebra, a remarkable feature is that, to fix the spin sites by boundaries through Bethe/Gauge, the spins of the sites will be reversed. This is similarly to the so called electron-hole effect, we call this as a boundary-spin effect, a new kind of duality.

==> ref.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% https://bibdesk.sourceforge.io/

%% Created for zhangting at 2023-11-22 18:46:24 +0800 


%% Saved with string encoding Unicode (UTF-8) 



@article{Gri17,
	author = {David J. Griffiths,},
	date-added = {2023-11-22 18:42:36 +0800},
	date-modified = {2023-11-22 18:46:23 +0800},
	journal = {Cambridge University Press},
	keywords = {doi:10.1017/9781108333511},
	title = {Introduction to Electrodynamics (4th ed.)},
	year = {2017}}

@article{SW97,
	author = {N. Seiberg and E. Witten},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {World Scientific, Singapore},
	title = {Gauge dynamics and compactification to three-dimensions, in The mathematical beauty of physics: A memorial volume for Claude Itzykson, C. Itzykson et al. Gauge dynamics and compactification to three-dimensions, in The mathematical beauty of physics: A memorial volume for Claude Itzykson, C. Itzykson et al.},
	volume = {arXiv:9607163},
	year = {1997}}

@article{NS09c,
	author = {N. Nekrasov and S. Shatashvili},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {arXiv:0908.4052},
	title = {QUANTIZATION OF INTEGRABLE SYSTEMS AND FOUR DIMENSIONAL GAUGE THEORIES}}

@article{DZ23b,
	abstract = {This note is an extension of [8] there the supersymmetric vacua of three-dimensional N=2 gauge theories with matter are shown to be in one-to-one correspondence with the eigenstate of XXZ integrable spin chain Hamiltonians with open boundary conditions. We consider the A2 quiver gauge theory, which is the simplest non-trivial quiver gauge theory, and sl3 open XXZ spin chain with diagonal boundary condition. We demonstrate the correspondence between the vacuum equations of different gauge groups and Bethe Ansatz equations with different boundary parameters. Not only that, but we furthermore push forward the program to the general Ar quiver gauge theory.},
	author = {Xiang-Mao Ding and Tinglyer Zhang},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	doi = {https://doi.org/10.1016/j.nuclphysb.2023.116222},
	issn = {0550-3213},
	journal = {Nuclear Physics B},
	pages = {116222},
	title = {Bethe/Gauge correspondence for linear quiver theories with ABCD gauge symmetry and spin chains},
	url = {https://www.sciencedirect.com/science/article/pii/S0550321323001517},
	volume = {991},
	year = {2023},
	bdsk-url-1 = {https://www.sciencedirect.com/science/article/pii/S0550321323001517},
	bdsk-url-2 = {https://doi.org/10.1016/j.nuclphysb.2023.116222}}

@article{DZ23a,
	abstract = {In this paper, we give a new effective superpotential that makes clear Bethe/Gauge correspondence between 2d (and 3d) SO/Sp gauge theories and open XXX (and XXZ) spin chains with diagonal boundary conditions, and also works in the case of 2d (and 3d) BCN-type gauge theories which is not previously discussed in the literature. Especially, for exceptional Lie algebras F4, G2, we give the effective superpotential and vacuum equations. For E6,7,8, we only give theirs effective superpotential for convenience.},
	author = {Ding, Xiang-Mao and Zhang, Tinglyer},
	date = {2023/04/06},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	doi = {10.1007/JHEP04(2023)036},
	id = {Ding2023},
	isbn = {1029-8479},
	journal = {Journal of High Energy Physics},
	number = {4},
	pages = {36},
	title = {Bethe/Gauge correspondence for ABCDEFG-type 3d gauge theories},
	url = {https://doi.org/10.1007/JHEP04(2023)036},
	volume = {2023},
	year = {2023},
	bdsk-url-1 = {https://doi.org/10.1007/JHEP04(2023)036}}

@article{SW94a,
	abstract = {We study the vacuum structure and don spectrum of N=2 supersymmetric gauge theory in four dimensions, with gauge group SU(2). The theory turns out to have remarkably rich and physical properties which can nonetheless be described precisely; exact formulas can be obtained, for instance, for electron and dyon masses and the metric on the moduli space of vacua. The description involves a version of Olive-Montonen electric-magnetic duality. The ``strongly coupled'' vacuum turns out to be a weakly coupled theory of monopoles, and with a suitable perturbation confinement is described by monopole condensation.},
	author = {N. Seiberg and E. Witten},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	doi = {https://doi.org/10.1016/0550-3213(94)90124-4},
	issn = {0550-3213},
	journal = {Nuclear Physics B},
	number = {1},
	pages = {19-52},
	title = {Electric-magnetic duality, monopole condensation, and confinement in N=2 supersymmetric Yang-Mills theory},
	url = {https://www.sciencedirect.com/science/article/pii/0550321394901244},
	volume = {426},
	year = {1994},
	bdsk-url-1 = {https://www.sciencedirect.com/science/article/pii/0550321394901244},
	bdsk-url-2 = {https://doi.org/10.1016/0550-3213(94)90124-4}}

@article{SW94b,
	abstract = {We study four dimensional N = 2 supersymmetric gauge theories with matter multiplets. For all such models for which the gauge group is SU(2), we derive the exact metric on the moduli space of quantum vacua and the exact spectrum of the stable massive states. A number of new physical phenomena occur, such as chiral symmetry breaking that is driven by the condensation of magnetic monopoles that carry global quantum numbers. For those cases in which conformal invariance is broken only by mass terms, the formalism automatically gives results that are invariant under electric-magnetic duality. In one instance, this duality is mixed in an interesting way with SO(8) triality.},
	author = {N. Seiberg and E. Witten},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	doi = {https://doi.org/10.1016/0550-3213(94)90214-3},
	issn = {0550-3213},
	journal = {Nuclear Physics B},
	number = {3},
	pages = {484-550},
	title = {Monopoles, duality and chiral symmetry breaking in N = 2 supersymmetric QCD},
	url = {https://www.sciencedirect.com/science/article/pii/0550321394902143},
	volume = {431},
	year = {1994},
	bdsk-url-1 = {https://www.sciencedirect.com/science/article/pii/0550321394902143},
	bdsk-url-2 = {https://doi.org/10.1016/0550-3213(94)90214-3}}

@article{KZ21,
	abstract = {In this article, we extend the work of {$[$}1{$]$} to a Bethe/Gauge correspondence between 2d (or resp. 3d) SO/Sp gauge theories and open XXX (resp. XXZ) spin chains with diagonal boundary conditions. The case of linear quiver gauge theories is also considered.},
	author = {Kimura, Taro and Zhu, Rui-Dong},
	date = {2021/03/24},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	doi = {10.1007/JHEP03(2021)227},
	id = {Kimura2021},
	isbn = {1029-8479},
	journal = {Journal of High Energy Physics},
	number = {3},
	pages = {227},
	title = {Bethe/gauge correspondence for SO/Sp gauge theories and open spin chains},
	url = {https://doi.org/10.1007/JHEP03(2021)227},
	volume = {2021},
	year = {2021},
	bdsk-url-1 = {https://doi.org/10.1007/JHEP03(2021)227}}

@article{NN21,
	author = {Lee, N., Nekrasov, N.},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {Journal of High Energy Physics},
	number = {93},
	title = {Quantum spin systems and supersymmetric gauge theories. Part I.},
	volume = {2021},
	year = {2021},
	bdsk-url-1 = {https://doi.org/10.1007/JHEP03(2021)093}}

@article{NPS18,
	abstract = {We study macroscopically two dimensional {\$}{\$}{\{}{$\backslash$}mathcal{\{}N{\}}=(2,2){\}}{\$}{\$}supersymmetric gauge theories constructed by compactifying the quiver gauge theories with eight supercharges on a product {\$}{\$}{\{}{$\backslash$}mathbb{\{}T{\}}\^{}{\{}d{\}} {$\backslash$}times {$\backslash$}mathbb{\{}R{\}}\^{}{\{}2{\}}{\_}{\{}{$\backslash$}epsilon{\}}{\}}{\$}{\$}of a d-dimensional torus and a two dimensional cigar with {\$}{\$}{\{}{$\backslash$}Omega{\}}{\$}{\$}-deformation. We compute the universal part of the effective twisted superpotential. In doing so we establish the correspondence between the gauge theories and the Yangian {\$}{\$}{\{}{$\backslash$}mathbf{\{}Y{\}}{\_}{\{}{$\backslash$}epsilon{\}}({$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}){\}}{\$}{\$}, quantum affine algebra {\$}{\$}{\{}{$\backslash$}mathbf{\{}U{\}}\^{}{\{}{$\backslash$}mathrm{\{}aff{\}}{\}}{\_}q({$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}){\}}{\$}{\$}, or the quantum elliptic algebra {\$}{\$}{\{}{$\backslash$}mathbf{\{}U{\}}\^{}{\{}{$\backslash$}mathrm{\{}ell{\}}{\}}{\_}{\{}q,p{\}}({$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}){\}}{\$}{\$}associated to Kac--Moody algebra {\$}{\$}{\{}{$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}{\}}{\$}{\$}for quiver {\$}{\$}{\{}{$\backslash$}Gamma{\}}{\$}{\$}.},
	author = {Nekrasov, Nikita and Pestun, Vasily and Shatashvili, Samson},
	date = {2018/01/01},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	doi = {10.1007/s00220-017-3071-y},
	id = {Nekrasov2018},
	isbn = {1432-0916},
	journal = {Communications in Mathematical Physics},
	number = {2},
	pages = {519--567},
	title = {Quantum Geometry and Quiver Gauge Theories},
	url = {https://doi.org/10.1007/s00220-017-3071-y},
	volume = {357},
	year = {2018},
	bdsk-url-1 = {https://doi.org/10.1007/s00220-017-3071-y}}

@article{YS20,
	author = {Yutaka Yoshida and Katsuyuki Sugiyama},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {Progress of Theoretical and Experimental Physics},
	number = {11},
	title = {Localization of three-dimensional N=2 supersymmetry theories on S1*D2},
	volume = {2020},
	year = {2020}}

@article{GKMMM95,
	abstract = {The exact Seiberg-Witten (SW) description of the light sector in the N = 2 SUSY 4d Yang-Mills theory [N. Seiberg and E. Witten, Nucl. Phys. B 430 (1994) 485 (E); B 446 (1994) 19] is reformulated in terms of integrable systems and appears to be a Gurevich-Pitaevsky (GP) [A. Gurevich and L. Pitaevsky, JETP 65 (1973) 65; see also, S. Novikov, S. Manakov, L. Pitaevsky and V. Zakharov, Theory of solitons] solution to the elliptic Whitham equations. We consider this as an implication that the dynamical mechanism behind the SW solution is related to integrable systems on the moduli space of instantons. We emphasize the role of the Whitham theory as a possible substitute of the renormalization-group approach to the construction of low-energy effective actions.},
	author = {A. Gorsky and I. Krichever and A. Marshakov and A. Mironov and A. Morozov},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	doi = {https://doi.org/10.1016/0370-2693(95)00723-X},
	issn = {0370-2693},
	journal = {Physics Letters B},
	number = {3},
	pages = {466-474},
	title = {Integrability and Seiberg-Witten exact solution},
	url = {https://www.sciencedirect.com/science/article/pii/037026939500723X},
	volume = {355},
	year = {1995},
	bdsk-url-1 = {https://www.sciencedirect.com/science/article/pii/037026939500723X},
	bdsk-url-2 = {https://doi.org/10.1016/0370-2693(95)00723-X}}

@article{NS09a,
	author = {N. Nekrasov and Samson L.Shatashvili},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {Nuclear Physics B},
	pages = {91--112},
	title = {Supersymmetric vacua and Bethe ansatz},
	volume = {192-193},
	year = {2009}}

@article{Hum72,
	author = {J.Humphreys},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	title = {Introduction to Lie Algebra and Representation Theory},
	year = {1972}}

@article{NS09b,
	author = {N. Nekrasov and Samson L.Shatashvili},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {AIP Conference Proceedings},
	pages = {154--169},
	title = {Bethe Ansatz and supersymmetric vacua},
	volume = {1134},
	year = {2009}}

@article{WYC15,
	author = {Y. Wang, W. L. Yang, J. Cao et al},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {Springer Berlin Heidelberg},
	title = {Off-diagonal Bethe Ansatz for exactly solvable models},
	year = {2015}}

@article{Bax07,
	author = {R. Baxter},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {Dover books onphysics},
	title = {Exactly Solved Models in Statistical Mechanics},
	year = {2007}}

@article{Fad96,
	author = {L. Faddeev},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {[arXiv:hep-th/9605187},
	title = {How algebraic Bethe ansatz works for integrable model},
	year = {1996}}

@article{NP23,
	author = {Nikita Nekrasov and Vasily Pestun},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {Symmetry, Integrability and Geometry: Methods and Applications},
	title = {Seiberg--Witten Geometry of Four-Dimensional N = 2 Quiver Gauge Theories},
	year = {2023}}

@article{FHSY96,
	author = {H. Fan, B.-Y. Hou, K.-J. Shi and Z.-X. Yang},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {Nucl. Phys. B 478 (1996) 723 [hep-th/9604016]},
	title = {Algebraic Bethe ansatz for eight vertex model with general open boundary conditions},
	year = {1996}}

@article{CK18,
	author = {Heng-Yu Chen and Taro Kimura},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {JHEP06(2018)165},
	title = {Quantum integrability from non-simply laced quiver gauge theory},
	year = {2018}}

@article{GK13,
	author = {Davide Gaiotto and Peter Koroteev},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {J. High Energ. Phys. 2013, 126 (2013},
	title = {On three dimensional quiver gauge theories and integrability},
	year = {2013}}

@article{NW21,
	author = {Hiraku Nakajima and Alex Weekes},
	date-added = {2023-10-18 16:38:49 +0800},
	date-modified = {2023-10-18 16:38:49 +0800},
	journal = {J. Eur. Math. Soc. 25, 203--230 (2023)},
	title = {Coulomb branches of quiver gauge theories with symmetrizers},
	year = {2021}}

@article{smaplearticle,
	archiveprefix = {arXiv},
	author = {First A.},
	doi = {DOI},
	eprint = {0000.0000},
	journal = {JHEP},
	pages = {PPP},
	title = {{Extended Theories of Gravity}},
	volume = {VV},
	year = {YYYY},
	bdsk-url-1 = {https://doi.org/DOI}}

